De-randomized PAC-Bayes Margin Bounds: Applications to Non-convex and Non-smooth Predictors

In spite of several notable efforts, explaining the generalization of deterministic non-smooth deep nets, e.g., ReLU-nets, has remained challenging. Existing approaches for deterministic non-smooth deep nets typically need to bound the Lipschitz constant of such deep nets but such bounds are quite large, may even increase with the training set size yielding vacuous generalization bounds. In this paper, we present a new family of de-randomized PAC-Bayes margin bounds for deterministic non-convex and non-smooth predictors, e.g., ReLU-nets. Unlike PAC-Bayes, which applies to Bayesian predictors, the de-randomized bounds apply to deterministic predictors like ReLU-nets. A specific instantiation of the bound depends on a trade-off between the (weighted) distance of the trained weights from the initialization and the effective curvature (`flatness') of the trained predictor. To get to these bounds, we first develop a de-randomization argument for non-convex but smooth predictors, e.g., linear deep networks (LDNs), which connects the performance of the deterministic predictor with a Bayesian predictor. We then consider non-smooth predictors which for any given input realized as a smooth predictor, e.g., ReLU-nets become some LDNs for any given input, but the realized smooth predictors can be different for different inputs. For such non-smooth predictors, we introduce a new PAC-Bayes analysis which takes advantage of the smoothness of the realized predictors, e.g., LDN, for a given input, and avoids dependency on the Lipschitz constant of the non-smooth predictor. After careful de-randomization, we get a bound for the deterministic non-smooth predictor. We also establish non-uniform sample complexity results based on such bounds. Finally, we present extensive empirical results of our bounds over changing training set size and randomness in labels.

==> app_aniso.tex <==

We consider the case where $\phi^{\theta}(x_i)$ is a smooth function of 
$\theta$, and provide detailed proofs of the technical results corresponding to PAC-Bayes 
with anisotropic posteriors briefly mentioned in Section~\ref{sec:margin2nc_updated}.


\subsection{Bounds for Stochastic vs.~Deterministic Predictors}

Recall Theorem~\ref{theo:s_marg} which establishes the relationship between stochastic and deterministic predictors in the main paper:
\theosmarg*

% As mentioned in Appendix~\ref{app:errata}, we also prove a deterministic version of Theorem~\ref{theo:s_marg} by essentially moving the bad probability $c_1 \exp(-\min(c_2 \tilde{\gamma}^2,c_3\tilde \gamma))$ to the right-hand-side of the bounds. The proofs of the two variants are essentially the same, with minor changes. For completeness, we state the deterministic version with exact constants. 


% \begin{theo}
% \label{theo:marg_sm_ani}
% Let $\sigma^2 > 0$ be chosen before seeing the training data.\footnote{More sophisticated choices of $\sigma^2$ are possible, e.g., based on using differential privacy~\citep{dzro18}, but we do not delve into such directions in the current paper.} Let $W$ be any distribution on pairs $(\x,y)$ with $\x \in \R^d$ and $y \in \{-1,+1\}$. For any $\theta^{\dagger} \in \R^d$, let $Q$ be a multivariate anisotropic Gaussian distribution with mean $\theta^{\dagger}$ and covariance $\Sigma_{\theta^{\dagger}}$, where 
% \begin{equation}
% \Sigma_{\theta^{\dagger}}^{-1} = \diag(\nu_1^2,\ldots,\nu_p^2)~,\qquad \nu_j^2 \triangleq \max \left\{ \cH_{l,\phi}^{\theta^{\dagger}}[j,j], \frac{1}{\sigma^2} \right\}~,
% \label{eq: cov_pos}
% \end{equation}
% where $\cH_{l,\phi}^{\theta^{\dagger}}$ is as in \eqref{eq:smooth_loss_hess}. Under Assumption~\ref{asmp:gen}, for any $\tilde \gamma > 2$ and any $\beta \in R$, we have 
% \begin{equation}
% \begin{split}
% \ell_{\beta}\left(Q, W\right) \leq \ell_{\beta + \sigma^2\alpha\tilde \gamma}(\phi^{\theta^{\dagger}},W) + 4\exp\left(- c\tilde \gamma\right)~,
% \label{eq:non_conv_marg_swd_ani}
% \end{split}
% \end{equation}
% and, 
% \begin{equation}
% \begin{split}
% \ell_{\beta}(\phi^{\theta^{\dagger}},W)  &\leq  \ell_{\beta + \sigma^2\alpha\tilde \gamma }(Q,W)+ 4\exp\left(- c\tilde \gamma\right)~,
% 	\label{eq:non_conv_marg_dws_ani}
% \end{split}
% \end{equation} 
% where $\alpha = \alpha_+ + \alpha_-$ and constant $c = c_0 \min\left[\frac{\sigma^2\alpha_+^2}{G^2},\frac{\sigma^2\alpha_-^2}{G^2},\frac{\alpha_+^2}{\eta_F^2}, \frac{\alpha_-^2}{\eta_F^2},\frac{\alpha_+}{\eta_2},\frac{\alpha_-}{\eta_2}\right]$, $c_0$ is an absolute constant. 
% \end{theo} 

% \begin{remark}
% Here the conditions $\tilde \gamma>1$ in Theorem~\ref{theo:s_marg} and $\tilde \gamma>2$ in Theorem~\ref{theo:marg_sm_ani} are applied for the same reason as discussed in Remark~\ref{rem:gamm_cond}.
% \end{remark}

First we prove the following result for anisotropic covariance $\delta \sim \cN(0,\Sigma_{\theta^\dagger})$ similar to Lemma~\ref{lemm: up_lo_H} for isotropic covariance $\delta\sim \cN(0,\sigma^2\I)$, which turns out to have the same bound:


\begin{lemm} \label{lemm: up_lo_H_ani}
For $\delta \sim \cN(0,\Sigma_{\theta^{\dagger}})$ and matrices $H_+, H_-$ are respectively positive and negative semi-definite with\\ $\max\left[\|H_-\|_F,\|H_+\|_F\right] \leq \eta_F, \max\left[\|H_-\|_2,\|H_+\|_2\right] \leq \eta_2$, and $\tr(H_+)\leq \alpha_+, \tr(H_-) \geq -\alpha_-$ for $\alpha_+, \alpha_- > 0$. We have the following upper bound and lower bound 
\begin{equation}
\begin{split}
    \P \left[  \delta^T H_- \delta   < -\sigma^2 \alpha_-\tilde \gamma  \right]  \leq  \exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{  \alpha_-(\tilde \gamma-1)}{ \eta_2} \right] \right)~,
    \label{eq:lb_h}
    \end{split}
\end{equation}
and
\begin{equation}
\begin{split}
    \P \left[  \delta^T H_+ \delta   >  \sigma^2 \alpha_+\tilde \gamma  \right]   \leq  \exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_+(\tilde \gamma-1)}{ \eta_2} \right] \right)~,
    \label{eq:ub_h}
    \end{split}
\end{equation}
where $\tilde \gamma >1$ and $c_0$ is an absolute constant.
\end{lemm}
\proof
Since $H_+$ is positive semi-definite, the diagonals of $H_+$ must be non-negative, then we have,
\begin{align*}
\E\left[\delta^TH_+\delta\right]=\E[\tr(H_+\delta\delta^T)]=\tr( H_+\Sigma_{\theta^{\dagger}}) &= \sum_i \min\left(\sigma^2, \frac{1}{\cH_{l,\phi}^{\theta^{\dagger}}[i,i]}\right) H_+[i,i]\\
 &   = \sigma^2 \sum_i \min\left(1, \frac{1}{\sigma^2 \cH_{l,\phi}^{\theta^{\dagger}}[i,i]}\right) H_+[i,i]\\
    & \leq \sigma^2 \sum_i H_+[i,i] = \sigma^2 \tr(H_+)\leq \sigma^2 \alpha_+~,
\end{align*}
Similarly, we have
\begin{align*}
\E\left[\delta^TH_-\delta\right]=\E[\tr(H_-\delta\delta^T)]=\tr( H_-\Sigma_{\theta^{\dagger}}) & = \sum_i \min\left(\sigma^2, \frac{1}{\cH_{l,\phi}^{\theta^{\dagger}}[i,i]}\right) H_-[i,i]\\
 &   = \sigma^2 \sum_i \min\left(1, \frac{1}{\sigma^2 \cH_{l,\phi}^{\theta^{\dagger}}[i,i]}\right) H_-[i,i]\\
    & \geq \sigma^2 \sum_i H_-[i,i] = \sigma^2 \tr(H_-)\geq -\sigma^2 \alpha_-~.
\end{align*}
We have
\begin{align}
\label{eq:psi2_ani}
    \kappa : = \max_i \|\delta_i\|_{\psi_2}\leq c_0 \max_i \min\left(\sigma, \frac{1}{\sqrt{\cH_{l,\phi}^{\theta^{\dagger}}[i,i]}}\right)\leq c_0\sigma~.
\end{align}
Therefore, from Hanson-Wright inequality we have
\begin{align*}
    \P\left[\delta^TH_+\delta-\sigma^2\alpha_+\geq t\right]\leq&\exp\left(-c_0\min\left[\frac{t^2}{\kappa^4\|H_+\|_F^2},\frac{t}{\kappa^2\|H_+\|_2}\right]\right)\\
    \leq &\exp\left(-c_0\min\left[\frac{t^2}{\kappa^4\eta_F^2},\frac{t}{\kappa^2\eta_2}\right]\right).
\end{align*}
By taking $t=\tilde \gamma\sigma^2 \alpha_+(>0)$, we have
\begin{equation}
\begin{split}
    \P[\delta^TH_+\delta\geq (\tilde \gamma+1)\sigma^2\alpha_+]\leq& \exp\left(-c_0\min\left[\frac{\sigma^4\alpha_+^2\tilde \gamma^2}{\kappa^4\eta_F^2},\frac{\sigma^2\alpha_+\tilde \gamma}{\kappa^2\eta_2}\right]\right)\\
    \leq &\exp\left(-c_0\min\left[\frac{\alpha_+^2\tilde \gamma^2}{\eta_F^2},\frac{\alpha_+\tilde \gamma}{\eta_2}\right]\right)~.
\end{split}
\end{equation}
Similarly, from Hanson-Wright inequality, we have
\begin{align*}
    \P\left[\delta^TH_-\delta-\sigma^2(-\alpha_-)\leq -t\right]\leq&\exp\left(-c_0\min\left[\frac{t^2}{\kappa^4\|H_-\|_F^2},\frac{t}{\kappa^2\|H_-\|_2}\right]\right)\\
    \leq&\exp\left(-c_0\min\left[\frac{t^2}{\kappa^4\eta_F^2},\frac{t}{\kappa^2\eta_2}\right]\right).
\end{align*}
Taking $t=\sigma^2\alpha_-\tilde \gamma(>0)$, we have
\begin{align}
    \P\left[\delta^TH_-\delta\leq -(\tilde \gamma+1)\sigma^2\alpha_-\right]    \leq& \exp\left(-c_0\min\left[\frac{\sigma^4\alpha_-^2\tilde \gamma^2}{\kappa^4\eta_F^2},\frac{\sigma^2\alpha_-\tilde \gamma}{\kappa^2\eta_2}\right]\right)\\
    \leq & \exp\left(-c_0\min\left[\frac{\alpha_-^2\tilde \gamma^2}{\eta_F^2},\frac{\alpha_-\tilde \gamma}{\eta_2}\right]\right).
\end{align}
Denote $\tilde \gamma+1$ as $\tilde \gamma$ completes the proof. \qed

{\em Proof of Theorem~\ref{theo:s_marg}:} Since $\phi$ is twice differentiable, for some suitable (random) $\tilde{\theta} = (1-\tau) \theta^{\dagger} + \tau \theta = \theta^{\dagger} + \tau (\theta - \theta^{\dagger})$ where $\tau \in [0,1]$, we have  

\begin{equation}
\phi^{\theta}(x_i) = \phi^{\theta^{\dagger}}(x_i) + \langle \theta - \theta^{\dagger}, \nabla \phi^{\theta^{\dagger}}(x_i) \rangle + \frac{1}{2} (\theta - \theta^{\dagger})^T H_{\phi}^{\tilde{\theta}}(x_i) (\theta - \theta^{\dagger})~. 
\end{equation}


%\subsection{Loss Bounds: Stochastic with Deterministic}
% We first establish \eqref{eq:non_conv_marg_swd_ani}. 
Consider the following set where $\theta^{\dagger}$ achieves a margin greater than $\left(\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma\right)$:

\begin{equation}
\cZ^{(>)}_{\beta + \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) = \bigg\{ (x,y) \in \cX \times \cY ~\bigg|~  y \phi^{\theta^{\dagger}}(x) > \beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~ \bigg\}~,
\end{equation}
where $\alpha = \alpha_- + \alpha_+$.

Let $P = \cN(0,\Sigma_{\theta^{\dagger}})$ be a multivariate distribution with mean 0 and covariance $\Sigma_{\theta^{\dagger}}$, where $\Sigma_{\theta^{\dagger}}$ is defined as \eqref{eq: cov_pos}. Now, for $z \in \cZ^{(>)}_{\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} )$, we have
\begin{align*}
\P_{\theta \sim \cQ}\bigg[ y \phi^{\theta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) \bigg] = \P_{\delta \sim P}\bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) \bigg] ~.
\end{align*}
Now, conditioned on $y =+1$, we have 
\begin{align*}
&\P_{\delta \sim P}\bigg[  \phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = +1 \bigg] \\
& = \P_{\delta \sim P}\bigg[  \phi^{\theta^{\dagger}}(x) + \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle +  \frac{1}{2}\delta^T H_{\phi}^{\tilde \theta}(x)  \delta \leq \beta ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma}(\theta^{\dagger}),  y = +1 \bigg] \\
& \leq  \P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle + \frac{1}{2}\delta^T H_-  \delta \leq \beta -\phi^{\theta^{\dagger}}(x)~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = +1 \bigg] \\
& \overset{(a)}{\leq}    \P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle + \frac{1}{2}\delta^T H_- \delta \leq -\frac{1}{2}\sigma^2 \tilde \gamma (\alpha_- +\alpha_+)~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = +1 \bigg]~ \\
& \overset{(b)}{\leq}    \P_{\delta \sim P}\bigg[\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle \leq -\frac{1}{2}\sigma^2 \alpha_+ \tilde \gamma ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = +1 \bigg] +\P_{\delta \sim P}\bigg[\delta^T H_- \delta \leq -\sigma^2 \alpha_-\tilde \gamma\bigg]~\\
% &\overset{(c)}{\leq}  \max_{z \in \cZ^{(>)}_{\beta + \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ),y=+1 }\P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle  \leq  -\sigma^2 \alpha_+ \tilde \gamma ~\big| z   \bigg]+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right) \\
& \overset{(c)}{\leq} \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)
\end{align*}

where (a) follows since for $(x,y) \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger})$ and $y=+1$ we have $\phi^{\theta^{\dagger}}(x) > \beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma$; (b) follows since $\P[x+y\leq a+b]\leq \P[x\leq a]+\P[y\leq b]$; (c) is from Hoeffding's inequality with $\| \nabla \phi^{\theta^{\dagger}}(x) \|_2^2 \leq G^2,~\max_i \|\delta_i\|_{\psi_2}\leq c_0 \sigma$, and Lemma \ref{lemm: up_lo_H_ani}.

Similarly, conditioned in $y =-1$, we have 
	\begin{align*}
&\P_{\delta \sim P}\bigg[  -\phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = -1 \bigg] \\
& = \P_{\delta \sim P}\bigg[  -\phi^{\theta^{\dagger}}(x) -\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle - \frac{1}{2}\delta^T H_{\phi}^{\tilde \theta}(x) \delta \leq \beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ),  y = -1 \bigg] \\
& \leq  \P_{\delta \sim P}\bigg[   -\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle - \frac{1}{2} \delta^T H_+ \delta \leq \beta + \phi^{\theta^{\dagger}}(x)~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = -1 \bigg] \\
& \overset{(a)}{\leq}    \P_{\delta \sim P}\bigg[   -\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle - \frac{1}{2}\delta^T H_+ \delta \leq -\frac{1}{2}\sigma^2  (\alpha_- +\alpha_+)\tilde \gamma  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = -1 \bigg]~ \\
& \overset{(b)}{\leq}    \P_{\delta \sim P}\bigg[   -\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle \leq -\frac{1}{2} \sigma^2 \alpha_- \tilde \gamma~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = -1 \bigg]+\P_{\delta \sim P}\bigg[ -\delta^T H_+ \delta\leq -\sigma^2\alpha_+ \tilde \gamma\bigg]~\\
% & \overset{(c)}{\leq}  \max_{z \in \cZ^{(>)}_{\beta + \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) }\P_{\delta \sim P}\bigg[   -\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle  \leq - \sigma^2 \alpha_- \tilde \gamma ~\big| z   \bigg]+ \exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)\\
& \overset{(c)}{\leq} \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)~,
\end{align*}
where (a) follows since for $(x,y) \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger})$ and $y=-1$ we have $-\phi^{\theta^{\dagger}}(x) > \beta + \sigma^2\alpha\tilde \gamma$; (b) follows since $\P[x+y\leq a+b]\leq \P[x\leq a]+\P[y\leq b]$; (c) is from Hoeffding's inequality with $\| \nabla \phi^{\theta^{\dagger}}(x) \|_2^2 \leq G^2,~\max_i \|\delta_i\|_{\psi_2}\leq c_0 \sigma$, and Lemma \ref{lemm: up_lo_H_ani}.

Then, we have

\begin{align*}
&\P_{\theta \sim \cQ}\bigg[ y \phi^{\theta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) \bigg]\\
&= \P_{\delta \sim P}\bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) \bigg] \\
& \leq   \P \bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ),  y = +1 \bigg]  + \P \bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = -1 \bigg] \\
& \leq \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)\\
&\quad+\exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)~.
\end{align*}
For $z \not \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} )$, we have
\begin{align*}
\P_{\theta \sim \cQ} \bigg[ y \phi^{\theta^\dagger}(x) ~\leq ~\beta  ~\big|~ z \not \in \cZ^{(>)}_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) \bigg] \leq 1 ~,
\end{align*}
By definition, we have
\begin{align*}
&\ell_{\beta}(\cQ,W)\\
& = \P_{\substack{\theta \sim \cQ\\ z \sim W}}\bigg[  y\phi^{\theta}(x) ~\leq ~\beta ~ \bigg] \\
& \leq    \P_{z \sim  W} \bigg[ y \phi^{\theta^{\dagger}}(x) \leq \beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma \bigg]+  \P_{\substack{\theta \sim \cQ\\ z \sim W}} \bigg[ y \phi^{\theta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma}(\theta^{\dagger}) \bigg] \\
& \leq   \P_{z \sim  W} \bigg[ y \phi^{\theta^{\dagger}}(x) \leq \beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma \bigg]+ \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right) \\
& \leq  \P_{z \sim  W} \bigg[ y \phi^{\theta^{\dagger}}(x) \leq \beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma \bigg]+ \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right) \\
& =  \ell_{\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma}(\phi^{\theta^{\dagger}},W)+ \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right) ~,
\end{align*}
which establishes \eqref{eq:s_aniso_swd}.


\label{sec: proof_dws}
Now we turn to the proof of  \eqref{eq:s_aniso_dws}. Consider the following set where $\theta^{\dagger}$ achieves a margin of at most $\beta$:
\begin{equation}
\cZ^{(\leq)}_{\beta}(\theta^{\dagger} ) = \bigg\{ (x,y) \in \cX \times \cY ~\bigg|~  y \phi^{\theta^{\dagger}}(x) \leq \beta ~ \bigg\}~.
\end{equation}

Let $P = \cN(0,\Sigma_{\theta^{\dagger}})$ be a multivariate distribution with mean 0 and covariance $\Sigma_{\theta^{\dagger}}$, where $\Sigma_{\theta^{\dagger}}$ is defined as \eqref{eq: cov_pos}. Now, for $z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger})$, we have
\begin{align*}
\P_{\theta \sim \cQ}\bigg[ y \phi^{\theta}(x) ~> ~ \beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}) \bigg]  = \P_{\delta \sim P}\bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~> ~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}) \bigg]~.
\end{align*}

Now, conditioned in $y =+1$, we have 
\begin{align*}
&\quad\P_{\delta \sim P}\bigg[  \phi^{\theta^{\dagger}+\delta}(x) ~> ~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}), y = +1 \bigg] \\
& = \P_{\delta \sim P}\bigg[  \phi^{\theta^{\dagger}}(x) + \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle +  \frac{1}{2}\delta^T H_{\phi}^{\tilde \theta}(x) \delta > \beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}),  y = +1 \bigg] \\
& \leq  \P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle + \frac{1}{2}\delta^T H_+ \delta > \beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma -\phi^{\theta^{\dagger}}(x)~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}),  y = +1 \bigg] \\
& \overset{(a)}{\leq}    \P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle + \frac{1}{2} \delta^T H_+ \delta > \frac{1}{2} \sigma^2\alpha\tilde \gamma~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}), y = +1 \bigg] \\
& \overset{(b)}{\leq}    \P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle  >  \frac{1}{2}\sigma^2\alpha_-\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}),  y = +1 \bigg]+\P_{\delta \sim P}\bigg[ \delta^T H_+ \delta \geq \frac{1}{2} \sigma \alpha_+ \tilde \gamma\bigg] \\
% & \overset{(c)}{\leq}  \max_{z \in \cZ^{(>)}_{\beta }(\theta^{\dagger} ) }\P_{\delta \sim P}\bigg[   \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle  > \sigma^2 \alpha_- \tilde \gamma~\big| z   \bigg] + \exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)\\
& \overset{(c)}{\leq} \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)~,
\end{align*}
where (a) follows since for $(x,y) \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger})$ and $y=+1$ we have $\phi(\theta^{\dagger}) \leq \beta \Rightarrow \beta -\phi(\theta) \geq 0$;  (b) follows since $\P[x+y\leq a+b]\leq \P[x\leq a]+\P[y\leq b]$; (c) is from Hoeffding's inequality with $\| \nabla \phi^{\theta^{\dagger}}(x) \|_2^2 \leq G^2,~\max_i \|\delta_i\|_{\psi_2}\leq c_0 \sigma$, and Lemma \ref{lemm: up_lo_H_ani}.

Similarly, conditioned on $y =-1$, we have 
\begin{align*}
&\quad \P_{\delta \sim P}\bigg[  - \phi^{\theta^{\dagger}+\delta}(x) ~> ~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}), y = -1 \bigg] \\
& = \P_{\delta \sim P}\bigg[  - \phi^{\theta^{\dagger}}(x) - \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle -  \frac{1}{2} \delta^T H_{\phi}^{\tilde \theta}(x) \delta > \beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}),  y = -1 \bigg] \\
& \leq  \P_{\delta \sim P}\bigg[ -  \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle - \frac{1}{2} \delta^T H_- \delta > \beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma + \phi^{\theta^{\dagger}}(x)~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}), y = -1 \bigg] \\
& \overset{(a)}{\leq}    \P_{\delta \sim P}\bigg[ -  \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle - \frac{1}{2} \delta^T H_- \delta >   \frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}),  y = -1 \bigg] \\
& \overset{(b)}{\leq}    \P_{\delta \sim P}\bigg[   - \langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle  > \frac{1}{2}\sigma^2\alpha_+\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}), y = -1 \bigg]+ \P_{\delta \sim P}\bigg[-\delta^T H_-\delta \geq \sigma^2\alpha_- \tilde \gamma\bigg] \\
% & \overset{(c)}{\leq}  \max_{z \in \cZ^{(>)}_{\beta }(\theta^{\dagger} ) }\P_{\delta \sim P}\bigg[   -\langle \delta, \nabla \phi^{\theta^{\dagger}}(x) \rangle  >  \sigma^2 \alpha_+ \tilde \gamma ~\big| z   \bigg]+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right) \\
& \overset{(c)}{\leq} \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right),
\end{align*}
where (a) follows since for $(x,y) \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}$ and $y=-1$ we have $-\phi(\theta^{\dagger}) \leq \beta \Rightarrow \beta + \phi(\theta^{\dagger}) \geq 0$; (b) follows since $\P[x+y\leq a+b]\leq \P[x\leq a]+\P[y\leq b]$; (c) is from Hoeffding's inequality with $\| \nabla \phi^{\theta^{\dagger}}(x) \|_2^2 \leq G^2,~\max_i \|\delta_i\|_{\psi_2}\leq c_0 \sigma$, and Lemma \ref{lemm: up_lo_H_ani}.

Then, we have 
\begin{equation}
\begin{split}
&\P_{\theta \sim \cQ}\bigg[ y \phi^{\theta}(x) ~> ~\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma  ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}) \bigg]  \\
&= \P_{\delta \sim P}\bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~> ~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger})\bigg] \\
& \leq   \P \bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~> ~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}), y = +1 \bigg]+ \P \bigg[ y \phi^{\theta^{\dagger}+\delta}(x) ~>~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta }(\theta^{\dagger}),  y = -1 \bigg] \\
& \leq \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)\\
& \quad+\exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)~ .
\end{split}
\end{equation}
For $z \not \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger})$, we have
\begin{equation}
\begin{split}
\P_{\theta \sim \cQ}  \bigg[ y \phi^{\theta}(x) ~> ~\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma ~\big|~ z \not \in \cZ^{(\leq)}_{\beta }(\theta^{\dagger}) \bigg] \leq 1~.
\end{split}
\end{equation}
By definition, we have
\begin{equation}
\begin{split}
&1-  \ell_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma }(\cQ,W)\\
&= \P_{\substack{\theta \sim \cQ\\ z \sim W}}\bigg[  y\phi^{\theta}(x) ~> ~\beta +\frac{1}{2} \sigma^2\alpha\tilde \gamma ~ \bigg] \\
& \leq \P_{z \sim  W} \bigg[ y \phi^{\theta^{\dagger}}(x) > \beta  \bigg] +  \P_{\substack{\theta \sim \cQ\\ z \sim W}} \bigg[ y \phi^{\theta}(x) ~> ~\beta + \frac{1}{2} \sigma^2\alpha\tilde \gamma ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}) \bigg] \\
& \leq  \P_{z \sim  W} \bigg[ y \phi^{\theta^{\dagger}}(x) > \beta  \bigg]+ \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right) + \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right) \\
& \leq \P_{z \sim  W} \bigg[ y \phi^{\theta^{\dagger}}(x) > \beta  \bigg] + \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right) + \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right) \\
& = 1-\ell_{\beta}(\phi^{\theta^{\dagger}},W)  + \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right) + \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)~,
\end{split}
\end{equation}
which implies
\begin{equation}
\begin{split}
\ell_{\beta}&(\phi^{\theta^{\dagger}},W)  \leq  \ell_{\beta + \frac{1}{2}\sigma^2\alpha\tilde \gamma }(\cQ,W) + \exp \left( -c_0\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right) + \exp \left( -c_0\frac{\sigma^2 \alpha_-^2\tilde \gamma^2}{G^2} \right)\\
&\quad+\exp\left(- c_0 \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)+\exp\left(- c_0 \min \left[ \frac{ \alpha_+^2(\tilde \gamma-1)^2}{ \eta_F^2}, \frac{\alpha_+(\tilde \gamma-1)}{\eta_2} \right] \right)~.
\end{split}
\end{equation}
By choosing $\tilde \gamma>2$, we have  $(\tilde\gamma-1)^2 >\frac{1}{4} \tilde\gamma^2$, $\tilde\gamma - 1>\frac{1}{2}\tilde\gamma$, which completes the proof.  \qed


% The proof of Theorem~\ref{theo:s_marg} is a minor variant of the above proof, and we highlight the parts which need to change.

% {\em Proof of Theorem~\ref{theo:s_marg}:} The proof is essentially the same as Theorem~\ref{theo:marg_sm_ani} for the same reason as in the proof of Theorem~\ref{theo:marg_sm_non}. We have Lemma~\ref{lemm: up_lo_H_ani}, in the next step we bound $\P_{\theta \sim Q}\bigg[ y \phi^{\theta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ) \bigg]$ and $\P_{\theta \sim Q}\bigg[ y \phi^{\theta}(x) ~> ~\beta + \sigma^2\alpha\tilde \gamma  ~\big|~ z \in \cZ^{(\leq)}_{\beta}(\theta^{\dagger}) \bigg]$ with minor changes. Taking $\P_{\theta \sim Q}\bigg[ y \phi^{\theta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ),y=+1 \bigg]$ as an example,  we have with probability $  1- \exp\left(- c \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)$, the following holds
% 	\begin{equation}\begin{split}
% \P_{\delta \sim P}\bigg[  \phi^{\theta^{\dagger}+\delta}(x) ~\leq ~\beta  ~\big|~ z \in \cZ^{(>)}_{\beta + \sigma^2\alpha\tilde \gamma}(\theta^{\dagger} ), y = +1 \bigg]\leq \exp \left( -c\frac{\sigma^2 \alpha_+^2\tilde \gamma^2}{G^2} \right)
% \end{split}\end{equation}
% Similar changes apply for other cases, and the rest of the proof follows similar to the proof in Theorem~\ref{theo:marg_sm_ani}. In the last step, for $\tilde \gamma\geq 1+a $, we have for the high probability:
% \begin{align*}
%     1- \exp\left(- c \min \left[ \frac{ \alpha_-^2(\tilde \gamma-1)^2}{\eta_F^2}, \frac{ \alpha_-(\tilde \gamma-1)}{\eta_2} \right] \right)\geq 1- \exp\left(- c \min \left[ \frac{a^2}{(1+a)^2}\frac{ \alpha_-^2\tilde \gamma^2}{\eta_F^2}, \frac{a}{1+a}\frac{ \alpha_-\tilde \gamma}{\eta_2} \right] \right)~.
% \end{align*}
% Denoting $c_2 = \frac{a^2\alpha_-^2}{(1+a)^2\eta_F^2}$, $c_3 = \frac{a\alpha_-}{(1+a)\eta_2}$ completes the proof.
% \qed



\subsection{Deterministic Margin Bounds}
Recall Theorem~\ref{theo:smooth} which establishes the margin bound for deterministic smooth predictors in the main paper:
\theosmooth*

% As mentioned in Appendix~\ref{app:errata}, we also prove a uniform version of Theorem~\ref{theo:smooth} with the $\forall \theta^{\dagger}$ being inside the probability at least $(1-\delta)$. The proofs of the two variants are similar with minor changes, with the uniform version using Theorem~\ref{theo:marg_sm_ani} instead of Theorem~\ref{theo:s_marg} to relate the performance of deterministic and stochastic predictors. For completeness, we state the deterministic version with exact constants, and note that the same constants translate to Theorem~\ref{theo:smooth}.
% \begin{theo}
% \label{theo: bound_ani}
% Consider any $\theta_0 \in \R^p, \sigma^2 > 0$ chosen before training, and let $\theta^{\dagger}$ be the parameters of the model after training. Under Assumption \ref{asmp:gen}, with probability at least $1-\delta$, for any $\theta^{\dagger}$, let $\cH_{l,\phi}^{\theta^{\dagger}}$ be the Hessian as in \eqref{eq:smooth_loss_hess}. Let $\nu_j^2 = \max \left\{ \cH_{l,\phi}^{\theta^{\dagger}}[j,j],\frac{1}{\sigma^2} \right\}$,  $\tilde p = | \{ j : \cH_{l,\phi}^{\theta^{\dagger}}[j,j] > 1/ \sigma_j^2 \}|$, and  $\{ \tilde \nu_{(1)}, ..., \tilde \nu_{(\tilde p)}\}$ be the subset of values larger than $1/\sigma^2$, for any $\beta \in (0,1), \gamma > 4 \sigma^2 \alpha$, we have the following scale-invariant bound:
% \begin{align}
% \ell_{0}(\theta^{\dagger},D)  &\leq a_{\beta} \ell_{\gamma}(\theta^{\dagger},S) + 2c_0\exp\left( -c_4 \gamma \right) + 
% \frac{b_{\beta}}{2n} \left(  \underbrace{\sum_{\ell =1}^{\tilde p} \ln \frac{\tilde{\nu}^2_{(\ell)}}{1/\sigma^2}}_{\textup{effective curvature}}  +  \underbrace{\frac{\|\theta^{\dagger}-\theta_0\|_2^2}{\sigma^2}}_{\textup{$L_2$ norm}} \right) + b_{\beta} \frac{\log (\frac{1}{\delta})}{n}.
% \end{align}

% where $a_{\beta} = \frac{\log (1/\beta)}{1-\beta}, b_{\beta} = \frac{1}{1-\beta}$, $c_0 = 2(a_{\beta}+1)$, $c_4 = c \min\left[\frac{\alpha_+^2}{\alpha G^2},\frac{\alpha_-^2}{\alpha G^2},\frac{\alpha_+^2}{\sigma^2\alpha\eta_F^2}, \frac{\alpha_-^2}{\sigma^2\alpha\eta_F^2},\frac{\alpha_+}{\sigma^2\alpha\eta_2},\frac{\alpha_-}{\sigma^2\alpha\eta_2}\right]$, $G$, $\alpha_+$, $\alpha_-$, $\alpha$, $\eta_F$, $\eta_2$ are as in Assumption \ref{asmp:gen} and Theorem \ref{theo:marg_sm}, $c_4$ is an absolute constant.
% \end{theo}



\proof To get to a de-randomized margin bound, we utilize the results in Theorem~\ref{theo:s_marg}.
First, with $\beta = 0$,  $\sigma^2\tilde\gamma \alpha = \gamma$ and $W=D$ in Theorem~\ref{theo:s_marg}  we have
\begin{equation}
\begin{split}
\ell_0(\phi^{\theta^{\dagger}}, D)& \leq \ell_{\gamma/2}(\cQ,D) +    4\exp \left(-\min(c_2\frac{\gamma^2}{\sigma^4\alpha^2},c_1\frac{\gamma}{\sigma^2\alpha})\right)~.
\end{split}
\label{eq:dwsc_ani}
\end{equation}
Similarly, with $\beta = \gamma/2$ and $W=S$ in Theorem~\ref{theo:s_marg} we have
\begin{equation}
\begin{split}
\ell_{\gamma/2}(\cQ, S) &\leq \ell_{\gamma}(\phi^{\theta^{\dagger}},S) +   4\exp \left(-\min(c_2\frac{\gamma^2}{\sigma^4\alpha^2},c_1\frac{\gamma}{\sigma^2\alpha})\right)~.
\end{split}
\label{eq:swdc_ani}
\end{equation}

From the Fast Rate PAC-Bayesian bound \eqref{eq:fast_bayes}, with probability at least $(1-\delta)$ over the draw of $n$ samples $S \sim D^n$, for any $\beta \in (0,1)$ and for any $Q$ we have 
\begin{equation} \label{eq:pac_bound2}
    \ell_{\gamma/2}(Q,D) \leq \frac{\log (1/\beta)}{1-\beta} \ell_{\gamma/2}(Q,S) + \frac{1}{1 - \beta} \frac{ KL(Q \| P) + \log (\frac{1}{\delta}) }{n} ~,
\end{equation}

Noting that
\begin{align}%{ll}
	2KL(\cQ|| P) &= \sum_{j = 1}^{p} (\frac{1}{\sigma^2 \nu_j} -1)+ \sum_{j =1}^{p}\frac{|\theta[j]-\theta_0[j]|^2}{\sigma^2} + \sum_{i =1}^{p} \ln \frac{\nu_j}{1/\sigma^2} \nonumber\\
	& \leq \sum_{l =1}^{\tilde p} \ln \frac{\tilde \nu_{(l)}^2}{1/\sigma^2} +\frac{\|\theta^{\dagger}-\theta_0\|_2^2}{\sigma^2}, 
\end{align}
we have 
\begin{equation}
\begin{split}
\ell_{0}(\phi^{\theta^{\dagger}},D)  \leq \frac{\log (1/\beta)}{1-\beta} &\ell_{\gamma}(\phi^{\theta^{\dagger}},S) + 
\frac{1}{2(1 - \beta)} \left(  \sum_{\ell =1}^{\tilde p} \ln \frac{\tilde{\nu}^2_{(\ell)}}{1/\sigma^2}  +  \frac{\|\theta^{\dagger}-\theta_0\|_2^2}{\sigma^2} \right)\\
&+4\left(\frac{\log (1/\beta)}{1-\beta}+1\right)\exp \left(-\min(c_2\frac{\gamma^2}{\sigma^4\alpha^2},c_1\frac{\gamma}{\sigma^2\alpha})\right)+ \frac{1}{1 - \beta} \frac{\log (\frac{1}{\delta})}{n}.
\end{split}
\end{equation} 


Using the argument in the proof of Theorem \ref{theo: bound_iso}, we know that the $KL(Q\|P)$ in the PAC-Bayes bound \eqref{eq:pac_bound2} remains invariant under $\alpha$-scale transformation \citep{kl2011}, i.e., 
\begin{equation}
    KL(Q^\prime ||P^\prime) = KL(Q||P),
\end{equation}
where $Q^\prime$ and $P^\prime$ are the distributions after $\alpha$-scale transformation corresponding to $Q$ and $P$ respectively. 

Note that the other terms apart from the $KL(Q\|P)$ in \eqref{eq:pac_bound2} does not change by $\alpha$-scale transformation since the functions represented by  the networks are the same. 
Thus, our generalization bound is scale-invariant.
\qed

Our generalization bound  in Theorem \ref{theo:smooth} captures the information of local curvature by using the Hessian $\mathcal{H}_{l, \phi}^{\theta^{\dagger}}$ at the parameter $\theta^{\dagger}$. 
Recent work \citep{dipb17} show that the Hessian $\mathcal{H}_{l, \phi}^{\theta^{\dagger}}$ can be modified by a certain $\alpha$-scale transformation which scales the weights by non-negative coefficients but does not change the function. Thus, $\alpha$-scale transformation invalidates certain recently proposed flatness based generalization bounds \citep{hosc97b, kemn17} by arbitrarily changing the flatness of the loss landscape for deep networks. However, we show that our generalization bound which measure the generalization by the the KL divergence or differential relative entropy between the posterior and the prior distribution remains invariant,
although the although the local structure such as the Hessian $\mathcal{H}_{l, \phi}^{\theta^{\dagger}}$ 
get modified by the $\alpha$-scale transformation.
%with positively homogeneous activation 
%without changing the functions represented by the networks.

%Our generalization bound  \eqref{eq:pac-bound2} is based on the PAC-Bayes theorem which measure the generalization by the the KL divergence or differential relative entropy between the posterior and the prior distribution. \citet{kl2011} show that the KL-divergence between two continuous distributions remains invariant under invertible transformations, such as $\alpha$-scale transformation. Thus, the KL divergence between posterior and prior defined in Theorem \ref{theo:smooth} remains invariant,
%although the although the local structure such as the Hessian $\mathcal{H}_{l, \phi}^{\theta^{\dagger}}$ 
%get modified by the $\alpha$-scale transformation, which underlies our scale-invariant bound. 


%Recent work \citep{dipb17} show that the Hessian $\mathcal{H}_{l, \phi}^{\theta^{\dagger}}$ can be modified by a certain $\alpha$-scale transformation which scales the weights by non-negative coefficients but does not change the function. Thus, $\alpha$-scale transformation invalidates certain recently proposed flatness based generalization bounds \citep{hosc97b, kemn17} by arbitrarily changing the flatness of the loss landscape for deep networks
%with positively homogeneous activation 
%without changing the functions represented by the networks.

%Our generalization bound is build based on the PAC-Bayes theorem which measure the generalization by the the KL divergence or differential relative entropy between the posterior and the prior distribution. \citet{kl2011} show that the KL-divergence between two continuous distributions remains invariant under invertible transformations, such as $\alpha$-scale transformation. Thus, the posterior and prior defined in Theorem \ref{theo:smooth} remains invariant,
%although the although the local structure such as the Hessian $\mathcal{H}_{l, \phi}^{\theta^{\dagger}}$ 
%get modified by the $\alpha$-scale transformation, which underlies our scale-invariant bound. 





==> header.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\topmargin}{-1in}
\setlength{\oddsidemargin}{-1in}
\setlength{\textheight}{11in}
\setlength{\textwidth}{8.5in}
\setlength{\headheight}{0in}
\setlength{\headsep}{0in}
\addtolength{\topmargin}{2.5cm}
\addtolength{\oddsidemargin}{2.5cm}
\addtolength{\textheight}{-5cm}
\addtolength{\textwidth}{-5cm}

\setlength{\parindent}{0ex}
\setlength{\parskip}{3pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\setlength{\topmargin}{-5pt}
%\setlength{\oddsidemargin}{-30pt}
%\setlength{\evensidemargin}{-30pt}
%
%\setlength{\marginparwidth}{50pt}
%\setlength{\marginparsep}{5pt}
%
%\setlength{\textheight}{690pt}
%\setlength{\textwidth}{510pt}
%
%\setlength{\footskip}{45pt}
%
%\headheight  0.0truein
%\headsep     0.0truein



%\setlength{\unitlength}{1in}
%\footheight     0.15truein


%%%% % page settings
%%%% \setlength {\topmargin}{-0.5in}
%%%% \setlength {\textheight}{9in}
%%%% \setlength {\oddsidemargin}{-0.25truein}
%%%% \setlength {\evensidemargin}{-0.25truein}
%%%% %\setlength {\textwidth}{7in}
%%%% \setlength {\textwidth}{183.0mm}
%%%\setlength {\parskip}{3pt plus 1pt}
%%%
%%%%\topmargin      -16.0mm
%%%%\oddsidemargin  -11.0mm
%%%%\evensidemargin -11.0mm
%%%%\textheight     243.5mm
%%%%\textwidth      183.0mm
%%%% \columnsep        4.1mm
%%%% \parindent        1.0em
%%%% \headsep          6.3mm
%%%% \headheight        12pt
%%%% \lineskip           1pt
%%%% \normallineskip     1pt
%%%% \def\baselinestretch{1}
%%%
%%%
%%%\newfont{\mischead}{lcmssb8 scaled\magstephalf}
%%%
%%%\newcommand{\ls}[1]
%%%{
%%%  \dimen0=\fontdimen6\the\font
%%%  \lineskip=#1\dimen0
%%%  \advance\lineskip.5\fontdimen5\the\font
%%%  \advance\lineskip-\dimen0
%%%  \lineskiplimit=.9\lineskip
%%%  \baselineskip=\lineskip
%%%  \advance\baselineskip\dimen0
%%%  \normallineskip\lineskip
%%%  \normallineskiplimit\lineskiplimit
%%%  \normalbaselineskip\baselineskip
%%%  \ignorespaces
%%%  }
%%%
%%%
%%%
%%%
%%%%%%
%%%%%%  dubfigsingle.  2x1 double figure with only one \caption.
%%%%%%
%%%%%\newcommand{\dubfigsingle}[6]{
%%%%%\begin{figure}[t]
%%%%%\centerline{
%%%%%    \begin{minipage}{0.38\textwidth}
%%%%%      \begin{center}
%%%%%        \leavevmode
%%%%%        \setlength{\epsfxsize}{0.95\textwidth}
%%%%%        \epsffile{\Figdir#1}
%%%%%       \newline{\small (a) #2}
%%%%%      \end{center}
%%%%%    \end{minipage}
%%%%%    \begin{minipage}{0.38\textwidth}
%%%%%      \begin{center}
%%%%%        \leavevmode
%%%%%        \setlength{\epsfxsize}{0.975\textwidth}
%%%%%        \epsffile{\Figdir#3}
%%%%%       \newline{\small (b) #4}
%%%%%      \end{center}
%%%%%    \end{minipage}
%%%%%} \caption{#5}\label{fig:#6}
%%%%%%\hrule
%%%%%\end{figure}
%%%%%}

